From Words to Worth: Newborn Article Impact Prediction with LLM

As the academic landscape expands, the challenge of efficiently identifying impactful newly published articles grows increasingly vital. This paper introduces a promising approach, leveraging the capabilities of LLMs to predict the future impact of newborn articles solely based on titles and abstracts. Moving beyond traditional methods heavily reliant on external information, the proposed method employs LLM to discern the shared semantic features of highly impactful papers from a large collection of title-abstract pairs. These semantic features are further utilized to predict the proposed indicator, TNCSI_SP, which incorporates favorable normalization properties across value, field, and time. To facilitate parameter-efficient fine-tuning of the LLM, we have also meticulously curated a dataset containing over 12,000 entries, each annotated with titles, abstracts, and their corresponding TNCSI_SP values. The quantitative results, with an MAE of 0.216 and an NDCG@20 of 0.901, demonstrate that the proposed approach achieves state-of-the-art performance in predicting the impact of newborn articles when compared to several promising methods. Finally, we present a real-world application example for predicting the impact of newborn journal articles to demonstrate its noteworthy practical value. Overall, our findings challenge existing paradigms and propose a shift towards a more content-focused prediction of academic impact, offering new insights for article impact prediction.

==> tabs/application.tex <==
\begin{table}[ht]
    
    \begin{center}
        \begin{tabular}{p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
            \hline
            & A Set & B Set & C Set & D Set\\
            \hline
            \hline
            JCR & Q1 & Q2 & Q3 & Q4 \\
            \hline
            Top 5\% & \textbf{0.832}  &  0.763  & 0.690  & 0.676  \\
            \hline
            Top 25\% & 0.668  &  \textbf{0.671}  & 0.644  & 0.565  \\
            \hline


        \end{tabular}
    \end{center}
    \caption{Predicted TNCSI$_{\mathrm{SP}}$ values for journals in different JCR quartiles: Higher quartiles show higher predicted values. }
    \label{tab:application}
\end{table}

==> tabs/tab_abs_score.tex <==
\begin{table}[ht]
    
    \begin{center}
        \begin{tabular}{p{0.7\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
            \hline
            Abstract & $\hat{TNCSI}_{SP}$  & Description  \\
            \hline
            \hline
             Title\&Abstract & 0.216 & 0.901  \\
            \hline
            + Open Access Status  & 0.214 & 0.878  \\
            \hline
            + Release Dataset  & 0.212 & 0.915  \\
            \hline
            + SOTA Claim  & 0.215 & 0.881  \\
            \hline
            + RQM~\cite{zhao2024literature}   & 0.211 & \textbf{0.931}  \\
            \hline
            + All above  & \textbf{0.209} & 0.917  \\
            \hline

        \end{tabular}
    \end{center}
    \caption{Additional information improves prediction accuracy. 5xEXP}
    \label{tab:additional_info}
\end{table}

==> tabs/tab_addition_info.tex <==
\begin{table}[ht]
    
    \begin{center}
        \begin{tabular}{p{0.5\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
            \hline
            Input Type &  MAE↓ & NDCG↑  \\
            \hline
            \hline
             Title\&Abstract & 0.216 & 0.901  \\
            \hline
            + Open Access Status  & 0.214 & 0.878  \\
            \hline
            + Release Dataset  & 0.212 & 0.915  \\
            \hline
            + SOTA Claim  & 0.215 & 0.881  \\
            \hline
            + RQM~\cite{zhao2024literature}   & 0.211 & \textbf{0.931}  \\
            \hline
            + All above  & \textbf{0.209} & 0.917  \\
            \hline

        \end{tabular}
    \end{center}
    \caption{Additional information improves prediction accuracy. 5xEXP}
    \label{tab:additional_info}
\end{table}

==> tabs/tab_compare_with_others.tex <==
% \begin{table*}[ht]
    
%     \begin{center}
%         \begin{tabular}{p{0.40\linewidth}p{0.1\linewidth}p{0.05\linewidth}p{0.17\linewidth}p{0.17\linewidth}}
%             \hline
%              Methods & Target &  Lv. & NDCG (Reported) ↑& NDCG (@Lv. II) ↑  \\
%             \hline
%             \hline
%             MLP-based~\cite{ruan2020predicting} & Cites & I  & - & 0.618  \\
%             % (论文长度): (标题长度):(标题中的标点):(参考文献数量)(参考文献年龄) MLP
%             %\hline
%             LSTM-based~\cite{ma2021deep} & Cites & I  & 0.84 & 0.381 \\
%             % 只给摘要LSTM
%             %\hline
%             MLP-based~\cite{hu2023identifying} & Is Top 5\%? & I  & - & 0.629  \\ 
%             % 关键词数量 (Number of keywords)摘要长度 (Abstract length)论文长度 (Paper length)参考文献数量 (Number of references)
%             %\hline
%             MLP-based~\cite{abbas2023predicting} & Cites & I  & \textbf{0.95} & - \\
%             % 无法复现 仅依靠历史数据
%             %\hline
%             Model Ensemble~\cite{zhang2024predicting} & Cites & I  & - & 0.669  \\ 
%             % 根据cs.XX用多个MLP分类。
%             \hline
%             ChatGPT-based~\cite{de2024can} & Scores & II  & - & 0.051  \\
%             %\hline
%             LLM-based (\textit{ours}) & TNCSI$_\mathrm{\text{SP}}$ & II & 0.90 & \textbf{0.901} \\
%             \hline

%         \end{tabular}
%     \end{center}
%     \caption{Comparison with previous approaches: An upward arrow indicates that a higher value is better, and vice versa. Bold font denotes the best performance among all methods. A dash ``-'' is used to indicate that a value is not provided or not applicable. \rewrite{Check:} % 把Reported去掉，增加每个工作用了哪些信息的说明
%     }
%     \label{tab:comp_various_methods}
% \end{table*}


\begin{table*}[ht]
    
    \begin{center}
        \begin{tabular}{p{0.35\linewidth}p{0.03\linewidth}p{0.3\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
            \hline
             Methods & Lv. & Input Feature & Target  & NDCG ↑  \\
            \hline
            \hline
            MLP-based~\cite{ruan2020predicting}& I& paper length, reference numbers, etc.&Cites  & 0.618  \\
            % (论文长度): (标题长度):(标题中的标点):(参考文献数量)(参考文献年龄) MLP
            %\hline
            LSTM-based~\cite{ma2021deep} & I& title, and abstract & Cites  & 0.381 \\
            % 只给摘要LSTM
            %\hline
            MLP-based~\cite{hu2023identifying} & I & the same to~\cite{ruan2020predicting}  &  Is Top 5\%?  & 0.629  \\ 
            % 关键词数量 (Number of keywords)摘要长度 (Abstract length)论文长度 (Paper length)参考文献数量 (Number of references)
            Model Ensemble~\cite{zhang2024predicting}& I & ~\cite{ruan2020predicting} + research filed & Cites  & 0.669  \\ 
            % 根据cs.XX用多个MLP分类。
            \hline
            ChatGPT-based~\cite{de2024can} & II& abstract & Scores  & 0.051  \\
            %\hline
            Fine-tuned LLM-based (\textit{ours}) & II& title, and abstract & TNCSI$_\mathrm{\text{SP}}$  & \textbf{0.901} \\
            \hline

        \end{tabular}
    \end{center}
    \caption{Comparison with previous approaches: An upward arrow indicates that a higher value is better, and vice versa. Bold font denotes the best performance among all methods. A dash ``-'' is used to indicate that a value is not provided or not applicable.  % 把Reported去掉，增加每个工作用了哪些信息的说明 \rewrite{Check:}
    }
    \label{tab:comp_various_methods}
\end{table*}
% 说明统计学差异小于xxxzhang2024predicting,de2024can,
% 作者数量：每篇论文的作者数量。
% 关键词数量：作者定义的关键词数量。
% 摘要长度：摘要的字数。
% 论文长度：文章的页数。
% 引用数量：论文中引用的参考文献数量(main).

==> tabs/tab_diff_metrics.tex <==
\begin{table}[ht]
    
    \begin{center}
        \begin{tabular}{p{0.5\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
            \hline
             Target Metric &  MAE & NDCG  \\
            \hline
            \hline
            Cites$^{*}$    & - & 0.8  \\
            \hline
            TNCSI   & 0.3 & 0.8  \\
            \hline
            
            $TNCSI_{SP}$   & 0.3 & 0.8  \\
            \hline

        \end{tabular}
    \end{center}
    \caption{Superiority of the proposed $TNCSI_{SP}$. $^{*}$ denotes that MAE is not applicable for the cites metric.}
    \label{tab:diff_metrics}
\end{table}

% 说明统计学差异小于xxx

==> tabs/tab_diff_year_pub.tex <==
% \begin{table*}[ht]
%     \begin{center}
%         \begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
%             \hline
%             NAID & \multicolumn{2}{c}{Cites} & \multicolumn{2}{c}{TNCSI} & \multicolumn{2}{c}{TNCSI\_SP} \\
%             \cline{2-7}
%             & MAE & NDCG & MAE & NDCG & MAE & NDCG \\
%             \hline
%             \hline
%             2021  & 0.3 & 0.8 & 0.3 & 0.8 & 0.3 & 0.8 \\
%             \hline
%             2022  & 0.3 & 0.8 & 0.3 & 0.8 & 0.3 & 0.8 \\
%             \hline
%             2023  & 0.3 & 0.8 & 0.3 & 0.8 & 0.3 & 0.8 \\
%             \hline
%             ALL   & 0.3 & 0.8 & 0.3 & 0.8 & 0.3 & 0.8 \\
%             \hline
%         \end{tabular}
%     \end{center}
%     \caption{Performance of LLaMA3 on datasets from different years. Note that the training data for LLaMA3 extends only up to the very beginning of 2023.}
% \end{table*}

% \begin{table}[ht]
%     \begin{center}
%         \renewcommand{\arraystretch}{1.5} % 调整行高
%         \begin{tabular}{ccccc}
%             \hline
%             \multirow{2}{*}{NAID} & \multicolumn{2}{c}{TNCSI} & \multicolumn{2}{c}{TNCSI$_\mathrm{\text{SP}}$} \\
%             \cline{2-5}
%             & MAE & NDCG & MAE & NDCG \\
%             \hline
%             \hline
%             2020 & 0.269 & - & 0.229 & - \\ % 0.802 0.762
%             \hline
%             2021 & 0.313 & - & 0.241 & - \\ %0.691 0.684
%             \hline
%             2022 & 0.357 & - & 0.240 & - \\ %0.687 0.782
%             \hline
%             ALL & 0.302 & 0.864 & 0.216 & 0.901 \\
%             \hline
%         \end{tabular}
%     \end{center}
%     \caption{Performance of LLaMA3 on datasets from different years. 3xExp}
%     \label{tab:various_year}
% \end{table}

\begin{table}[ht]
    \begin{center}
        \renewcommand{\arraystretch}{1.5} % Adjusts row height
        \begin{tabular}{ccc}
            \hline
            Year & TNCSI & TNCSI$_\mathrm{\text{SP}}$ \\
            \hline
            \hline
            2020 & 0.269 & 0.229 \\
            \hline
            2021 & 0.313 & 0.241 \\
            \hline
            2022 & 0.357 & 0.240 \\
            \hline
            ALL & 0.302 & 0.216 \\
            \hline
        \end{tabular}
    \end{center}
    \caption{Performance of LLaMA3 on datasets from different years. 3xExp}
    \label{tab:various_year}
\end{table}



% Note that the training data for LLaMA3 extends only up to the very beginning of 2023.
% \begin{table*}[ht]
%     \begin{center}
%         \renewcommand{\arraystretch}{1.5} % 调整行高
%         \begin{tabular}{ccccccc}
%             \hline
%             \multirow{2}{*}{NAID} & \multicolumn{2}{c}{Cites$^{*}$} & \multicolumn{2}{c}{TNCSI} & \multicolumn{2}{c}{TNCSI\_SP} \\
%             \cline{2-7}
%             & MAE & NDCG & MAE & NDCG & MAE & NDCG \\
%             \hline
%             \hline
%             2021 & 0.3 & 0.8 & 0.3 & 0.8 & 0.3 & 0.8 \\
%             \hline
%             2022 & 0.3 & 0.8 & 0.3 & 0.8 & 0.3 & 0.8 \\
%             \hline
%             2023 & 0.3 & 0.8 & 0.3 & 0.8 & 0.3 & 0.8 \\
%             \hline
%             ALL & 0.3 & 0.8 & 0.3 & 0.8 & 0.3 & 0.8 \\
%             \hline
%         \end{tabular}
%     \end{center}
%     \caption{Performance of LLaMA3 on datasets from different years. Note that the training data for LLaMA3 extends only up to the very beginning of 2023. $^{*}$ denotes that MAE is not applicable for the cites metric.}
% \end{table*}


% 说明统计学差异小于xxx

==> tabs/tab_metric.tex <==
\begin{table}[ht]
    \renewcommand\arraystretch{1.1}
    \setlength{\tabcolsep}{4pt} % 调整表格内间距以节省空间
    \begin{center}
        \begin{tabular}{p{0.45\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
            \hline
            Bibliometric  &  Value & Field & Time\\ 
            \hline
            \hline
            Cites   & $\times$ & $\times$ & $\times$\\
            \hline
            FWCI~\cite{colledge2014snowball}   & $\times$ & \checkmark & $\times$\\
            \hline
            RCR~\cite{hutchins2016relative}  & $\times$ & \checkmark & $\times$\\
            \hline
            TNCSI~\cite{zhao2024literature}  & \checkmark & \checkmark & $\times$\\
            \hline
            TNCSI$_{\mathrm{SP}}$ (\textit{Ours})   & \checkmark & \checkmark & \checkmark\\
            \hline
        \end{tabular}
    \end{center}
    \caption{\textbf{Article-level Metrics for Evaluating Scholar Impact:} Value, field, and time respectively indicate whether the metric is a value between 0 and 1, whether it allows for cross-field comparisons, and whether it is suitable for the comparison of papers published at different times.}
    \label{tab:metric_compare}
\end{table}


==> tabs/tab_prompt_keyphrase.tex <==
\begin{table}[ht]
    \begin{center}
        \begin{tabular}{p{0.75\linewidth}p{0.1\linewidth}}
            \hline
             Prompt Template & NED↓ \\
            \hline
            \hline
             Identify the research field from the given title and abstract. You MUST respond with the keyword ONLY in this format: xxx  & 0.30 \\
            \hline
            Based on the title and abstract, determine the main area of study for the paper, focusing on a keyword that accurately represents the field. You MUST respond with the keyword ONLY in this format: xxx.  & 0.29 \\
            \hline
            Given the title and abstract below, determine the specific research field by focusing on the main application area and the key technology. You MUST respond with the keyword ONLY in this format: xxx.  & \textbf{0.26} \\
            \hline
        \end{tabular}
    \end{center}
    \caption{Effectiveness of prompt engineering: comparison of various user prompts for identifying key phrase.}
    \label{tab:tkpd_PE}
\end{table}

==> tabs/tab_prompt_predicting.tex <==
% \begin{table}[ht]

%     \begin{center}
%         \begin{tabular}{p{0.6\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
%             \hline
%              Prompt Template & MAE ↑ & NDCG ↓\\
%             \hline
%             \hline
%               Title: \{title\}, Abstract: \{abstract\}. & 0.067 & 0.75 \\
%             \hline
%              Given a certain paper entitled \{title\}, and its abstract: \{abstract\}. Predict its normalized scholar impact:    & 0.066 & x \\
%             \hline
%             Given a certain paper entitled \{title\}, and its abstract: \{abstract\}. Predict its normalized scholar impact (between 0 and 1):    & 0.216 & 0.901 \\
%             \hline
%             Given the provided title and abstract, predict the future normalized academic impact on a scale from 0 (lowest impact) to 1 (highest impact). You may consider factors such as the language clarity, novelty of the research, or the claim of state-of-the-art, etc. Title: \{title\} Abstract: \{abstract\}  & 0.216 & 0.901 \\
%             \hline

%         \end{tabular}
%     \end{center}
%     \caption{Effectiveness of prompt engineering: comparison of various user prompts. This experiment trains for only ten epochs. 2xEXP}
%     \label{tab:llm_PE}
% \end{table}

\begin{table}[ht]

    \begin{center}
        \begin{tabular}{p{0.75\linewidth}p{0.12\linewidth}}
            \hline
             Prompt Template & NDCG↑\\
            \hline
            \hline
              Title: \{title\}, Abstract: \{abstract\}. & 0.849  \\
            \hline

            Given the provided title and abstract, predict the future normalized academic impact on a scale from 0 (lowest impact) to 1 (highest impact). You may consider factors such as the language clarity, novelty of the research, or the claim of state-of-the-art, etc. Title: \{title\} Abstract: \{abstract\}  & 0.869  \\
            \hline
             Given a certain paper entitled \{title\}, and its abstract: \{abstract\}. Predict its normalized scholar impact:    & 0.889  \\
            \hline
            Given a certain paper entitled \{title\}, and its abstract: \{abstract\}. Predict its normalized scholar impact (between 0 and 1):    & \textbf{0.901} \\

            \hline

        \end{tabular}
    \end{center}
    \caption{Effectiveness of prompt engineering: comparison of various prompts for guilding LLMs to predict the future impact. }
    \label{tab:llm_PE}
\end{table}

==> tabs/tab_various_LLM_compare.tex <==
\begin{table}[ht]

    \renewcommand\arraystretch{1.1}

    \begin{center}
    
        \begin{tabular}{cccccc}
            \hline
            LLMs & Size ↓ & MAE ↓ & NDCG ↑ & Memory ↓ \\
            \hline
            \hline
            Phi-3& \textbf{3.8B}& 0.226 & 0.742 & \textbf{6.2GB}  \\
            %\hline
             Falcon& 7B& 0.231 & 0.740 & 8.9GB\\
             %\hline
             Qwen-2 & 7B  & 0.223 & 0.774 & 12.6GB  \\
             %\hline
            Mistral& 7B & 0.220 & 0.850 & 15.4GB  \\
             %\hline

             LLama-3 & 8B & \textbf{0.216}  &  \textbf{0.901} & 9.4GB  \\

            \hline
        \end{tabular}
    
    \end{center}
    \caption{Performance Comparison of Different LLM Models on the NAID test set: size refers to the number of model parameters, and memory stands for the minimum memory usage during inference.}
    \label{tab:various_LLM_compare}
\end{table}
